How to Inverting the Leverage Score Distribution?

Leverage score is a fundamental problem in machine learning and theoretical computer science. It has extensive applications in regression analysis, randomized algorithms, and neural network inversion. Despite leverage scores are widely used as a tool, in this paper, we study a novel problem, namely the inverting leverage score problem. We analyze to invert the leverage score distributions back to recover model parameters. Specifically, given a leverage score $\sigma \in \mathbb{R}^n$, the matrix $A \in \mathbb{R}^{n \times d}$, and the vector $b \in \mathbb{R}^n$, we analyze the non-convex optimization problem of finding $x \in \mathbb{R}^d$ to minimize $\| \mathrm{diag}( \sigma ) - I_n \circ (A(x) (A(x)^\top A(x) )^{-1} A(x)^\top ) \|_F$, where $A(x):= S(x)^{-1} A \in \mathbb{R}^{n \times d} $, $S(x) := \mathrm{diag}(s(x)) \in \mathbb{R}^{n \times n}$ and $s(x) : = Ax - b \in \mathbb{R}^n$. Our theoretical studies include computing the gradient and Hessian, demonstrating that the Hessian matrix is positive definite and Lipschitz, and constructing first-order and second-order algorithms to solve this regression problem. Our work combines iterative shrinking and the induction hypothesis to ensure global convergence rates for the Newton method, as well as the properties of Lipschitz and strong convexity to guarantee the performance of gradient descent. This important study on inverting statistical leverage opens up numerous new applications in interpretation, data recovery, and security.

==> main_result.tex <==


\section{Main Result}
\label{sec:main}

In this section, we present our main result.


\begin{theorem}[Formal version of Theorem~\ref{thm:main_informal}]\label{thm:main_formal}
If the following conditions hold:
    \begin{itemize}
        \item Let $A \in \R^{n \times d}$.
        \item Let $b \in \R^n$.
        \item Let $\sigma \in \R^n$.
        \item Let $s(x) \in \R^n$.
        \item Let $S(x) := \diag(s(x)) \in \R^{n \times n}$.
        \item Let $A(x):= S(x)^{-1} A \in \R^{n \times d}$. 
        \item Let $\epsilon > 0$.
    \end{itemize}
    
     Then, we have
     \begin{itemize}
         \item {\bf Part 1.} there exists an algorithm (see Algorithm~\ref{alg:first_order}), which uses the first order iteration and runs in $O( \epsilon^{-1} {l^2}/{\alpha} ) $ (where $l = 812 \beta^{-9}R^5$ from Lemma~\ref{lem:lipschitz_informal}, $\alpha = \sigma_{\min}(D) \cdot \sigma_{\min}(A)^2 > 0$ from Lemma~\ref{lem:convex}) iterations and spends ??
    time per iteration and solves the inverting leverage score problem (defined in Definition~\ref{def:inverting_leverage_score}):
    \begin{align*}
        \min_{x \in \R^d } \| \diag( \sigma ) - I_n \circ (A(x) (A(x)^\top A(x) )^{-1} A(x)^\top )  \|_F.
    \end{align*}
    and finally outputs $x_T$ such that
    \begin{align*}
        L(x_T) - L(x^*) < \epsilon.
    \end{align*}
    with probability $1 - \poly(n)$. 
    \item {\bf Part 2.} there exists an algorithm (see Algorithm~\ref{alg:second_order}), which uses the second order iteration and runs in $\log(r_0/\epsilon)$ iterations and spends 
    \begin{align*}
        \wt O(n^4 + \Tmat (n,n,n))
    \end{align*}
    time per iteration and solves the inverting leverage score problem (defined in Definition~\ref{def:inverting_leverage_score}):
    \begin{align*}
        \min_{x \in \R^d } \| \diag( \sigma ) - I_n \circ (A(x) (A(x)^\top A(x) )^{-1} A(x)^\top )  \|_F.
    \end{align*}
    and finally outputs $x_T$ such that
    \begin{align*}
        \|x_T - x^*\|_2 < \epsilon
    \end{align*}
    with probability $1 - \poly(n)$. 
     \end{itemize}
\end{theorem}

\begin{proof}
    {\bf Proof of the number of iterations.}

    {\bf Part 1} follows from Lemma~\ref{lem:gradient_convergence}, and {\bf Part 2} follows from Lemma~\ref{lem:newton_induction}.

    {\bf Proof of gradient computation.}

    This follows from Lemma~\ref{lem:gradient_leverage_informal}, which takes
    \begin{align*}
        \Tmat (n,n,n) 
    \end{align*}
    time.

    {\bf Proof of Hessian computation.}
    
    This follows from calling Lemma~\ref{lem:hessian_decompose_informal} for $n$ times, which takes
    \begin{align*}
        n \cdot ( \Tmat(n,d,d)  + O(n^4) ) 
    \end{align*}
    time.

    {\bf Proof of Hessian Being Positive Definite.}
    

    This follows from Lemma~\ref{lem:convex_informal}.
    


    {\bf Proof of Hessian Being Lipschitz.}

    This follows from Lemma~\ref{lem:lipschitz_informal}.
\end{proof}
